Prompt Diffusion Robustifies Any-Modality Prompt Learning

Foundation models enable prompt-based classifiers for zero-shot and few-shot learning. Nonetheless, the conventional method of employing fixed prompts suffers from distributional shifts that negatively impact generalizability to unseen samples. This paper introduces prompt diffusion, which uses a diffusion model to gradually refine the prompts to obtain a customized prompt for each sample. Specifically, we first optimize a collection of prompts to obtain over-fitted prompts per sample. Then, we propose a prompt diffusion model within the prompt space, enabling the training of a generative transition process from a random prompt to its overfitted prompt. As we cannot access the label of a test image during inference, our model gradually generates customized prompts solely from random prompts using our trained, prompt diffusion. Our prompt diffusion is generic, flexible, and modality-agnostic, making it a simple plug-and-play module seamlessly embedded into existing prompt learning methods for textual, visual, or multi-modal prompt learning. Our diffusion model uses a fast ODE-based sampling strategy to optimize test sample prompts in just five steps, offering a good trade-off between performance improvement and computational efficiency. For all prompt learning methods tested, adding prompt diffusion yields more robust results for base-to-new generalization, cross-dataset generalization, and domain generalization in classification tasks tested over 15 diverse datasets.

==> images/framework.tex <==
\begin{figure}[t]
  \begin{subfigure}{0.49\textwidth}
    \includegraphics[width=0.9\linewidth]{images/train_fw_7.pdf}
    \caption{\textbf{Training phase: forward diffusion and reverse denoising.}}
  \end{subfigure}
  \hspace{1cm}
  \begin{subfigure}{0.49\textwidth}
    \includegraphics[width=0.85\linewidth]{images/test_fw_8.pdf}
    \caption{\textbf{Testing phase: diffusion sampling. }}
  \end{subfigure}
  \caption{\textbf{Diffusion prompting}.
In the \textit{training} phase (a), we begin by generating prompts that are initially overfitted using per-sample overfitting. These prompts are then subjected to a noise injection step before entering the forward diffusion process. The inputs for diffusion include the noisy prompts $\tilde{\bm{V}_t^*}$, the image features $\pi$, and a randomly chosen time step $t$, leading to the generation of diffused prompts $\tilde{\bm{V}_t}$. Upon completing the training, the diffusion transformer acquires the capability to convert generic prompts into their overfitted counterparts for each sample.
%
In the \textit{testing} phase (b), the sampling process begins with an initial random noise $\tilde{\bm{V}}_{T}$, which is gradually refined into diffused prompts $\tilde{\bm{V}}{t}$. At each time step $t$, the sampling process incorporates the previous state $\tilde{\bm{V}}_{t-1}$, the test image features $\pi$, and the current time step $t$ as inputs. The resulting diffused prompts $\tilde{\bm{V}_0}$ are then employed for making predictions on test samples. Throughout $T$ time steps with our diffusion transformer, the vanilla prompts are adapted into customized prompts that contain more specific information about the test sample, thereby enhancing prediction accuracy.
}
 \label{fig:framework}
 \vspace{-5mm}
\end{figure}


==> images/uncertainty.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.85\linewidth]{images/uncer_diff_1.pdf}
    \vspace{-0.5em}
    \caption{\textbf{Effect of Monte Carlo sampling} on base-to-new generalization. Increasing samples improves accuracy at the cost of an increased time complexity at inference. We observe a good trade-off for 50 samples.}
    \vspace{-6mm}
    \label{fig:uncertainty}
\end{figure}

==> tables/algo_prograd.tex <==
\begin{figure}[t]
\begin{minipage}[t]{\linewidth}
\centering
     \begin{minipage}[t]{0.5\linewidth}
          \begin{figure}[H]
              \includegraphics[width=0.99\linewidth]{images/ProGrad.pdf}
              \caption{(a): if $\bm{g}_\text{ce}$ is aligned with $\bm{g}_\text{kl}$, we set $\bm{g}_\text{prograd}$ as $\bm{g}_\text{ce}$. (b): if $\bm{g}_\text{ce}$ conflicts with $\bm{g}_\text{kl}$ (\ie, their angle is larger than 90\degree), we set $\bm{g}_\text{prograd}$ as the projection of $\bm{g}_\text{ce}$ on the vertical direction of $\bm{g}_\text{kl}$.}
              \label{fig:conflict}
          \end{figure}
      \end{minipage}
    \hspace{2mm}
    \begin{minipage}[t]{0.4\linewidth}
        \begin{algorithm}[H]
        \caption{Prompt-aligned Gradient}\label{alg:projgrad}
        \begin{algorithmic}[1]
        \Require Learnable context $\bm{v}$, zero-shot CLIP prediction $\bm{y}_\text{zs}$, ground-truth label $\bm{y}_\text{gt}$, learning rate $\alpha$.
        \State $\bm{g}_\text{ce}\gets \nabla_{\bm{v}}\mathcal{L}_\text{ce}(\bm{v})$
        \State $\bm{g}_\text{kl}\gets \nabla_{\bm{v}}\mathcal{L}_\text{kl}(\bm{v})$
        \If{ $\bm{g}_\text{ce} \cdot \bm{g}_\text{kl}$ $\geq$ 0} 
            \State $\bm{g}_\text{prograd}\gets \bm{g}_\text{ce}$
        \Else
            \State $\bm{g}_\text{prograd} \gets  \bm{g}_\text{ce} - \frac{\bm{g}_\text{ce} \cdot \bm{g}_\text{kl}}{\|\bm{g}_\text{kl}\|^2}\bm{g}_\text{kl}  $ 
        \EndIf
        \State $\bm{v} \gets \bm{v}-\alpha\cdot \bm{g}_\text{prograd} $
        \end{algorithmic}
        \end{algorithm}
    \end{minipage}
    %
 
\end{minipage}
\end{figure}

==> tables/base2new.tex <==
\begin{table}[t]
	\tabstyle{1pt}
 	\caption{\textbf{Base-to-new generalization.} Prompts are derived from base class examples. The harmonic mean (H) underscores the trade-off in generalization. Top-performing results are emphasized in \textbf{\color{blue}blue}. 
 %
    By integrating our plugin within three different prompt learning methods, we consistently improve their average accuracy across 11 datasets, demonstrating enhanced performance over approaches without our plugin. }
	\vspace{-0.7mm}
 	\begin{subtable}[t]{.24\textwidth}
		\centering
		\caption{\textbf{Average}}
		    \scalebox{.65}{
		\begin{tabular}{l cc|c}
			\toprule
			& Base & New & H \\
			\midrule
			CLIP & 69.34 & 74.22 & 71.70 \tikzmark{start1a}\\
			CoOp    &77.58  &73.11  &75.28   \tikzmark{end1a}\\
			\midrule
			VPT   &72.53  &72.34  &72.43  \tikzmark{start1a} \\
               \rowcolor{lightGray}
			{+ \textit{Ours}}   &{74.98}  &{74.97}  &{75.03} \tikzmark{end1a} \\
			\midrule
                   CoCoOp &{80.47} & 71.69 &75.83 \tikzmark{start1a}\\
                                \rowcolor{lightGray}
			{+ \textit{Ours}}   &{81.35}  &{74.97}  &{77.72}  \tikzmark{end1a}\\
			\midrule
         MaPLe & 82.28 & {75.14} & {78.55}  \tikzmark{start1a}\\
                      \rowcolor{lightGray}
			{+ \textit{Ours}}   &\color{blue}\textbf{{83.39}}  &\color{blue}\textbf{77.32}  &\color{blue}\textbf{80.36}  \tikzmark{end1a} \\         
			\bottomrule
		\end{tabular}}
    \begin{tikzpicture}[overlay, remember picture, dashed, black]
    \draw[line width=0.3pt,rectangle,rounded corners]
        ($(pic cs:start1a) + (-4.2cm, 3.5cm)$) rectangle 
        ($(pic cs:end1a) + (-1.4cm, 0.5cm)$);
\end{tikzpicture}
	\end{subtable}
	\vspace{-0.7mm}
	\begin{subtable}[t]{.24\textwidth}
		\centering
		\caption{ImageNet.}
		    \scalebox{.65}{
		\begin{tabular}{l cc|c}
			\toprule
			& Base & New & H \\
			\midrule
			CLIP & 72.43 & 68.14 & 70.22 \\
   			CoOp    &76.21 &69.98   &72.96   \\
			\midrule
			VPT   &74.45  &69.22  &71.74   \\
           \rowcolor{lightGray}
			{+ \textit{Ours}}   &{74.97}  &{69.99}  &{72.97}   \\
			\midrule
   			CoCoOp & 75.98 &70.43 &73.10 \\
              \rowcolor{lightGray}
			{+ \textit{Ours}}   &{76.46}  &{70.97} &{73.36}   \\
			\midrule
    MaPLe & {76.66} & {70.54} & {73.47} \\
            \rowcolor{lightGray}
    			{+ \textit{Ours}}   & \color{blue}\textbf{77.01}  &\color{blue}\textbf{71.03}  &\color{blue}\textbf{74.25}   \\
			\bottomrule
		\end{tabular}}
	\end{subtable}
	~\vspace{-0.7mm}
	\begin{subtable}[t]{.24\textwidth}
		\centering
		\caption{Caltech101.}
		    \scalebox{.65}{
		\begin{tabular}{l cc|c}
			\toprule
			& Base & New & H \\
			\midrule
			CLIP & 96.84 &94.00 & 95.40 \\
   			CoOp     &97.49   &94.67   &96.06   \\
			\midrule 
			VPT   &96.92  &93.44  &95.15   \\
			 \rowcolor{lightGray} {+ \textit{Ours}}  &{97.43}  &{94.23}  &{95.83}    \\
			\midrule
      			CoCoOp & 97.96 & 93.81 & 95.84 \\
			 \rowcolor{lightGray} {+ \textit{Ours}}   &\color{blue}\textbf{98.12} &{94.97}  &{96.48}   \\
			\midrule
    MaPLe & 97.74 & {94.36} & {96.02} \\
    			 \rowcolor{lightGray} {+ \textit{Ours}}   &{97.25}  & \color{blue}\textbf{95.98}  &\color{blue}\textbf{96.81}   \\
			\bottomrule
		\end{tabular}}
	\end{subtable}
\vspace{-0.7mm}
	\begin{subtable}[t]{.24\textwidth}
		\centering
		\caption{OxfordPets.}
			  \scalebox{.65}{
		\begin{tabular}{l cc|c}
			\toprule
			& Base & New & H \\
			\midrule
			CLIP & 91.17 & 97.26 & 94.12 \\
   			CoOp    &94.48  & 95.88 &95.17   \\
			\midrule
			VPT   &92.63  &94.96  &93.78   \\
			 \rowcolor{lightGray} {+ \textit{Ours}}   &{93.17}  &{97.18}  &{95.64}    \\
			\midrule
      			CoCoOp &{95.20} & 97.69 &{96.43} \\
			 \rowcolor{lightGray} {+ \textit{Ours}}   &{94.97}  &{97.98}  &{96.97}   \\
			\midrule
    MaPLe & {95.43} & {97.76} & {96.58} \\
    			 \rowcolor{lightGray} {+ \textit{Ours}}   &\color{blue}\textbf{95.96}  &\color{blue}\textbf{98.11}  &\color{blue}\textbf{97.36}   \\
			\bottomrule
		\end{tabular}}
	\end{subtable}
	\vspace{-0.7mm}

	\begin{subtable}[t]{.24\textwidth}
		\centering
		\caption{StanfordCars.}
			  \scalebox{.65}{
		\begin{tabular}{l cc|c}
			\toprule
			& Base & New & H \\
			\midrule
			CLIP & 63.37 & 74.89 & 68.65 \\
   			CoOp    &71.26  &73.92  &72.57   \\
			\midrule
   			VPT   &65.06  &74.68  &69.54   \\
			 \rowcolor{lightGray} {+ \textit{Ours}}   &{65.75}  &{75.23}  &{70.96}   \\
			\midrule
      			CoCoOp & 70.49 & 73.59 & 72.01 \\
			 \rowcolor{lightGray} {+ \textit{Ours}}   &{70.98}  &\color{blue}\textbf{75.32}  &\color{blue}\textbf{74.11}  \\
			\midrule
    MaPLe & 72.94 & 74.00 & {73.47} \\
    			 \rowcolor{lightGray} {+ \textit{Ours}}   &\color{blue}\textbf{73.11}  &{75.03}  &{74.06}   \\
			\bottomrule
		\end{tabular}}
	\end{subtable}\vspace{-0.7mm}
	\begin{subtable}[t]{.24\textwidth}
		\centering
		\caption{Flowers102.}
					  \scalebox{.65}{
		\begin{tabular}{l cc|c}
			\toprule
			& Base & New & H \\
			\midrule
			CLIP & 72.08 & 77.80 & 74.83 \\
   			CoOp    &87.87  &74.11  &80.41   \\
			\midrule
   			VPT   &76.23  &71.55  &73.82   \\
			 \rowcolor{lightGray} {+ \textit{Ours}}   &{77.29}  &{72.33}  &{74.71}    \\
			\midrule
      			CoCoOp & 94.87 & 71.75 & 81.71 \\
			 \rowcolor{lightGray} {+ \textit{Ours}}   &{94.17}  &\color{blue}\textbf{75.73}  &\color{blue}\textbf{83.32}   \\
			\midrule
    MaPLe & 95.92 & 72.46 & {82.56} \\
    			 \rowcolor{lightGray} {+ \textit{Ours}}   &\color{blue}\textbf{95.90}  &{73.14}  &{83.07}   \\
			\bottomrule
		\end{tabular}}
	\end{subtable}\vspace{-0.7mm}
	\begin{subtable}[t]{.24\textwidth}
		\centering
		\caption{Food101.}
					  \scalebox{.65}{
		\begin{tabular}{l cc|c}
			\toprule
			& Base & New & H \\
			\midrule
			CLIP & 90.10 & 91.22 & 90.66 \\
   			CoOp    &90.63  &91.17  &90.90   \\
			\midrule
			VPT   &89.27  &90.50  &89.88   \\
			 \rowcolor{lightGray} {+ \textit{Ours}}   &{89.97}  &{92.12}  &{91.03}   \\
			\midrule
      			CoCoOp & 90.70 & 91.29 & 90.99 \\
			 \rowcolor{lightGray} {+ \textit{Ours}}   &{90.21}  &{92.01}  &{91.38}   \\
			\midrule
    MaPLe & {90.71} & {92.05} & {91.38} \\
    			 \rowcolor{lightGray} {+ \textit{Ours}}   &\color{blue}\textbf{91.26}  &\color{blue}\textbf{93.11}  &\color{blue}\textbf{92.17}   \\
			\bottomrule
		\end{tabular}}
	\end{subtable}\vspace{-0.7mm}
	\begin{subtable}[t]{.24\textwidth}
		\centering
		\caption{FGVCAircraft.}
					  \scalebox{.65}{
		\begin{tabular}{l cc|c}
			\toprule
			& Base & New & H \\
			\midrule
			CLIP & 27.19 & 36.29 & 31.09 \\
   			CoOp    &30.66  &35.73  &33.00   \\
			\midrule
   			VPT   &28.23  &32.21  &30.09   \\
			 \rowcolor{lightGray} {+ \textit{Ours}}   &{28.82}  &{35.07}  &{32.01}    \\
			\midrule
      			CoCoOp &{33.41} & 23.71 & 27.74 \\
			 \rowcolor{lightGray} {+ \textit{Ours}}   &{34.21}  &{35.27}  &{33.61}   \\
			\midrule
    MaPLe & 37.44 & 35.61 & {36.50} \\
    			 \rowcolor{lightGray} {+ \textit{Ours}}   &\color{blue}\textbf{37.11}  &\color{blue}\textbf{36.15}  &\color{blue}\textbf{36.43}   \\
			\bottomrule
		\end{tabular}}
	\end{subtable}
	~\vspace{-0.7mm}


 
	\begin{subtable}[t]{.24\textwidth}
		\centering
		\caption{SUN397.}
					  \scalebox{.65}{
		\begin{tabular}{l cc|c}
			\toprule
			& Base & New & H \\
			\midrule
			CLIP & 69.36 & 75.35 & 72.23 \\
   			CoOp    &79.78  &76.04  &77.87   \\
			\midrule
			VPT   &75.14  &76.89  &76.00   \\
			 \rowcolor{lightGray} {+ \textit{Ours}}   &{75.74}  &{77.82}  &{76.93} \\
			\midrule
      			CoCoOp & 79.74 & 76.86 & 78.27\\
			 \rowcolor{lightGray} {+ \textit{Ours}}   &{80.14}  &{77.53}  &{79.11}   \\
			\midrule
    MaPLe & {80.82} & {78.70} & {79.75} \\
    			 \rowcolor{lightGray} {+ \textit{Ours}}   &\color{blue}\textbf{81.03}  &\color{blue}\textbf{79.54}  &\color{blue}\textbf{80.01}   \\
			\bottomrule
		\end{tabular}}
	\end{subtable}\vspace{-0.7mm}
	\begin{subtable}[t]{.24\textwidth}
		\centering
		\caption{DTD.}
					  \scalebox{.65}{
		\begin{tabular}{l cc|c}
			\toprule
			& Base & New & H \\
			\midrule
			CLIP & 53.24 & 59.90 & 56.37 \\
   			CoOp    &69.46  &55.67  &61.81   \\
			\midrule
   			VPT   &56.71  &57.25  &56.98   \\
			 \rowcolor{lightGray} {+ \textit{Ours}}  &{58.43}  &{58.13}  &{58.65}  \\
			\midrule
      			CoCoOp &{77.01} & 56.00 & 64.85 \\
			 \rowcolor{lightGray} {+ \textit{Ours}}   &{73.43}  &{60.19}  &{65.91}   \\
			\midrule
    MaPLe & \color{blue}\textbf{80.36} & 59.18 & {68.16} \\
    			 \rowcolor{lightGray} {+ \textit{Ours}}   &{80.25}  &\color{blue}\textbf{59.94}  &\color{blue}\textbf{68.25}   \\
			\bottomrule
		\end{tabular}}
	\end{subtable}\vspace{-0.7mm}
	\begin{subtable}[t]{.24\textwidth}
		\centering
		\caption{EuroSAT.}
					  \scalebox{.65}{
		\begin{tabular}{l cc|c}
			\toprule
			& Base & New & H \\
			\midrule
			CLIP & 56.48 & 64.05 & 60.03 \\
   			CoOp    &74.79  &61.50  &67.50   \\
			\midrule
   			VPT   &67.57  &59.69  &63.39   \\
			+ \textit{Ours}  &{67.26}  &{69.01}  &{72.81}  \\
			\midrule
      			CoCoOp & {87.49} & 60.04 & 71.21 \\
			+ \textit{Ours}  &{88.13}  &{70.22}  &{72.97}   \\
			\midrule
    MaPLe & {94.07} & {73.23} & \color{blue}\textbf{82.35} \\
    			 \rowcolor{lightGray} {+ \textit{Ours}}   &\color{blue}\textbf{94.76}  &\color{blue}\textbf{73.34}  &{82.96}   \\
			\bottomrule
		\end{tabular}}
	\end{subtable}\vspace{-0.7mm}
	\begin{subtable}[t]{.24\textwidth}
		\centering
		\caption{UCF101.}
					  \scalebox{.65}{
		\begin{tabular}{l cc|c}
			\toprule
			& Base & New & H \\
			\midrule
			CLIP & 70.53 & 77.50 & 73.85 \\
   			CoOp    &80.72  &75.55  &78.05   \\
			\midrule
   			VPT   &75.65  &75.31  &75.48   \\
			 \rowcolor{lightGray} {+ \textit{Ours}}   &{76.31}  &{76.23}  &{76.66}  \\
			\midrule
   			CoCoOp & {82.33} & 73.45 & 77.64 \\
			 \rowcolor{lightGray} {+ \textit{Ours}}   &{81.97}  &{77.03}  &{79.21}   \\
			\midrule
    MaPLe & \color{blue}\textbf{83.00} & {78.66} & \color{blue}\textbf{80.77} \\
    			 \rowcolor{lightGray} {+ \textit{Ours}}   &{82.86}  &\color{blue}\textbf{79.64}  &{80.73}   \\
			\bottomrule
		\end{tabular}}
	\end{subtable}
	~\vspace{-8mm}
  \label{tab:base2new}
\end{table}




% \begin{table}[t]
% 	\tabstyle{1pt}
%  	\caption{\textbf{Base-to-new generalization.} Prompts are derived from base class examples. The harmonic mean (H) underscores the trade-off in generalization. Top-performing results are emphasized in \textbf{\color{blue}blue}. 
%  %
%     By integrating our plugin within three different prompt learning methods, we consistently improve their average accuracy across 11 datasets, demonstrating enhanced performance over approaches without our plugin. }
% 	\vspace{-1mm}
%  	\begin{subtable}[t]{.32\textwidth}
% 		\centering
% 		\caption{\textbf{Average}}
% 		    \scalebox{.6}{
% 		\begin{tabular}{l cc|c}
% 			\toprule
% 			& Base & New & H \\
% 			\midrule
% 			CLIP~\cite{radford2021learning} & 69.34 & 74.22 & 71.70 \\
% 			CoOp~\cite{COOP}   &77.58  &73.11  &75.28   \\
% 			\midrule
% 			VPT~\cite{jia2022visual}   &72.53  &72.34  &72.43   \\
%                \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &{74.98}  &{74.97}  &{75.03}  \\
% 			\midrule
%                    CoCoOp~\cite{cocoop} &{80.47} & 71.69 &75.83 \\
%                                 \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &{81.35}  &{74.97}  &{77.72}  \\
% 			\midrule
%          MaPLe~\cite{khattak2023maple} & 82.28 & {75.14} & {78.55}  \\
%                       \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &\color{blue}\textbf{{83.39}}  &\color{blue}\textbf{77.32}  &\color{blue}\textbf{80.36}   \\         
% 			\bottomrule
% 		\end{tabular}}
% 	\end{subtable}
% 	\vspace{-1mm}
% 	\begin{subtable}[t]{.32\textwidth}
% 		\centering
% 		\caption{ImageNet.}
% 		    \scalebox{.6}{
% 		\begin{tabular}{l cc|c}
% 			\toprule
% 			& Base & New & H \\
% 			\midrule
% 			CLIP~\cite{radford2021learning} & 72.43 & 68.14 & 70.22 \\
%    			CoOp~\cite{COOP}   &76.21 &69.98   &72.96   \\
% 			\midrule
% 			VPT~\cite{jia2022visual}   &74.45  &69.22  &71.74   \\
%            \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &{74.97}  &{69.99}  &{72.97}   \\
% 			\midrule
%    			CoCoOp~\cite{cocoop} & 75.98 &70.43 &73.10 \\
%               \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &{76.46}  &{70.97} &{73.36}   \\
% 			\midrule
%     MaPLe~\cite{khattak2023maple} & {76.66} & {70.54} & {73.47} \\
%             \rowcolor{lightGray}
%     			{+ {Prompt Diffusion}}   & \color{blue}\textbf{77.01}  &\color{blue}\textbf{71.03}  &\color{blue}\textbf{74.25}   \\
% 			\bottomrule
% 		\end{tabular}}
% 	\end{subtable}
% 	~\vspace{-1mm}
% 	\begin{subtable}[t]{.32\textwidth}
% 		\centering
% 		\caption{Caltech101.}
% 		    \scalebox{.6}{
% 		\begin{tabular}{l cc|c}
% 			\toprule
% 			& Base & New & H \\
% 			\midrule
% 			CLIP~\cite{radford2021learning} & 96.84 &94.00 & 95.40 \\
%    			CoOp~\cite{COOP}    &97.49   &94.67   &96.06   \\
% 			\midrule 
% 			VPT~\cite{jia2022visual}   &96.92  &93.44  &95.15   \\
% 			 \rowcolor{lightGray} {+ {Prompt Diffusion}}  &{97.43}  &{94.23}  &{95.83}    \\
% 			\midrule
%       			CoCoOp~\cite{cocoop} & 97.96 & 93.81 & 95.84 \\
% 			 \rowcolor{lightGray} {+ {Prompt Diffusion}}   &\color{blue}\textbf{98.12} &{94.97}  &{96.48}   \\
% 			\midrule
%     MaPLe~\cite{khattak2023maple} & 97.74 & {94.36} & {96.02} \\
%     			 \rowcolor{lightGray} {+ {Prompt Diffusion}}   &{97.25}  & \color{blue}\textbf{95.98}  &\color{blue}\textbf{96.81}   \\
% 			\bottomrule
% 		\end{tabular}}
% 	\end{subtable}
% \vspace{-1mm}
%  	\begin{subtable}[t]{.32\textwidth}
% 		\centering
% 		\caption{\textbf{Average}}
% 		    \scalebox{.6}{
% 		\begin{tabular}{l cc|c}
% 			\toprule
% 			& Base & New & H \\
% 			\midrule
% 			CLIP~\cite{radford2021learning} & 69.34 & 74.22 & 71.70 \\
% 			CoOp~\cite{COOP}   &77.58  &73.11  &75.28   \\
% 			\midrule
% 			VPT~\cite{jia2022visual}   &72.53  &72.34  &72.43   \\
%                \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &{74.98}  &{74.97}  &{75.03}  \\
% 			\midrule
%                    CoCoOp~\cite{cocoop} &{80.47} & 71.69 &75.83 \\
%                                 \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &{81.35}  &{74.97}  &{77.72}  \\
% 			\midrule
%          MaPLe~\cite{khattak2023maple} & 82.28 & {75.14} & {78.55}  \\
%                       \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &\color{blue}\textbf{{83.39}}  &\color{blue}\textbf{77.32}  &\color{blue}\textbf{80.36}   \\         
% 			\bottomrule
% 		\end{tabular}}
% 	\end{subtable}
% 	\vspace{-1mm}
% 	\begin{subtable}[t]{.32\textwidth}
% 		\centering
% 		\caption{ImageNet.}
% 		    \scalebox{.6}{
% 		\begin{tabular}{l cc|c}
% 			\toprule
% 			& Base & New & H \\
% 			\midrule
% 			CLIP~\cite{radford2021learning} & 72.43 & 68.14 & 70.22 \\
%    			CoOp~\cite{COOP}   &76.21 &69.98   &72.96   \\
% 			\midrule
% 			VPT~\cite{jia2022visual}   &74.45  &69.22  &71.74   \\
%            \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &{74.97}  &{69.99}  &{72.97}   \\
% 			\midrule
%    			CoCoOp~\cite{cocoop} & 75.98 &70.43 &73.10 \\
%               \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &{76.46}  &{70.97} &{73.36}   \\
% 			\midrule
%     MaPLe~\cite{khattak2023maple} & {76.66} & {70.54} & {73.47} \\
%             \rowcolor{lightGray}
%     			{+ {Prompt Diffusion}}   & \color{blue}\textbf{77.01}  &\color{blue}\textbf{71.03}  &\color{blue}\textbf{74.25}   \\
% 			\bottomrule
% 		\end{tabular}}
% 	\end{subtable}
% 	~\vspace{-1mm}
% 	\begin{subtable}[t]{.32\textwidth}
% 		\centering
% 		\caption{Caltech101.}
% 		    \scalebox{.6}{
% 		\begin{tabular}{l cc|c}
% 			\toprule
% 			& Base & New & H \\
% 			\midrule
% 			CLIP~\cite{radford2021learning} & 96.84 &94.00 & 95.40 \\
%    			CoOp~\cite{COOP}    &97.49   &94.67   &96.06   \\
% 			\midrule 
% 			VPT~\cite{jia2022visual}   &96.92  &93.44  &95.15   \\
% 			 \rowcolor{lightGray} {+ {Prompt Diffusion}}  &{97.43}  &{94.23}  &{95.83}    \\
% 			\midrule
%       			CoCoOp~\cite{cocoop} & 97.96 & 93.81 & 95.84 \\
% 			 \rowcolor{lightGray} {+ {Prompt Diffusion}}   &\color{blue}\textbf{98.12} &{94.97}  &{96.48}   \\
% 			\midrule
%     MaPLe~\cite{khattak2023maple} & 97.74 & {94.36} & {96.02} \\
%     			 \rowcolor{lightGray} {+ {Prompt Diffusion}}   &{97.25}  & \color{blue}\textbf{95.98}  &\color{blue}\textbf{96.81}   \\
% 			\bottomrule
% 		\end{tabular}}
% 	\end{subtable}
%  	~\vspace{-1mm}
%   	\begin{subtable}[t]{.32\textwidth}
% 		\centering
% 		\caption{\textbf{Average}}
% 		    \scalebox{.6}{
% 		\begin{tabular}{l cc|c}
% 			\toprule
% 			& Base & New & H \\
% 			\midrule
% 			CLIP~\cite{radford2021learning} & 69.34 & 74.22 & 71.70 \\
% 			CoOp~\cite{COOP}   &77.58  &73.11  &75.28   \\
% 			\midrule
% 			VPT~\cite{jia2022visual}   &72.53  &72.34  &72.43   \\
%                \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &{74.98}  &{74.97}  &{75.03}  \\
% 			\midrule
%                    CoCoOp~\cite{cocoop} &{80.47} & 71.69 &75.83 \\
%                                 \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &{81.35}  &{74.97}  &{77.72}  \\
% 			\midrule
%          MaPLe~\cite{khattak2023maple} & 82.28 & {75.14} & {78.55}  \\
%                       \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &\color{blue}\textbf{{83.39}}  &\color{blue}\textbf{77.32}  &\color{blue}\textbf{80.36}   \\         
% 			\bottomrule
% 		\end{tabular}}
% 	\end{subtable}
% 	\vspace{-1mm}
% 	\begin{subtable}[t]{.32\textwidth}
% 		\centering
% 		\caption{ImageNet.}
% 		    \scalebox{.6}{
% 		\begin{tabular}{l cc|c}
% 			\toprule
% 			& Base & New & H \\
% 			\midrule
% 			CLIP~\cite{radford2021learning} & 72.43 & 68.14 & 70.22 \\
%    			CoOp~\cite{COOP}   &76.21 &69.98   &72.96   \\
% 			\midrule
% 			VPT~\cite{jia2022visual}   &74.45  &69.22  &71.74   \\
%            \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &{74.97}  &{69.99}  &{72.97}   \\
% 			\midrule
%    			CoCoOp~\cite{cocoop} & 75.98 &70.43 &73.10 \\
%               \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &{76.46}  &{70.97} &{73.36}   \\
% 			\midrule
%     MaPLe~\cite{khattak2023maple} & {76.66} & {70.54} & {73.47} \\
%             \rowcolor{lightGray}
%     			{+ {Prompt Diffusion}}   & \color{blue}\textbf{77.01}  &\color{blue}\textbf{71.03}  &\color{blue}\textbf{74.25}   \\
% 			\bottomrule
% 		\end{tabular}}
% 	\end{subtable}
% 	~\vspace{-1mm}
% 	\begin{subtable}[t]{.32\textwidth}
% 		\centering
% 		\caption{Caltech101.}
% 		    \scalebox{.6}{
% 		\begin{tabular}{l cc|c}
% 			\toprule
% 			& Base & New & H \\
% 			\midrule
% 			CLIP~\cite{radford2021learning} & 96.84 &94.00 & 95.40 \\
%    			CoOp~\cite{COOP}    &97.49   &94.67   &96.06   \\
% 			\midrule 
% 			VPT~\cite{jia2022visual}   &96.92  &93.44  &95.15   \\
% 			 \rowcolor{lightGray} {+ {Prompt Diffusion}}  &{97.43}  &{94.23}  &{95.83}    \\
% 			\midrule
%       			CoCoOp~\cite{cocoop} & 97.96 & 93.81 & 95.84 \\
% 			 \rowcolor{lightGray} {+ {Prompt Diffusion}}   &\color{blue}\textbf{98.12} &{94.97}  &{96.48}   \\
% 			\midrule
%     MaPLe~\cite{khattak2023maple} & 97.74 & {94.36} & {96.02} \\
%     			 \rowcolor{lightGray} {+ {Prompt Diffusion}}   &{97.25}  & \color{blue}\textbf{95.98}  &\color{blue}\textbf{96.81}   \\
% 			\bottomrule
% 		\end{tabular}}
% 	\end{subtable}
%  	~\vspace{-1mm}
%   	\begin{subtable}[t]{.32\textwidth}
% 		\centering
% 		\caption{\textbf{Average}}
% 		    \scalebox{.6}{
% 		\begin{tabular}{l cc|c}
% 			\toprule
% 			& Base & New & H \\
% 			\midrule
% 			CLIP~\cite{radford2021learning} & 69.34 & 74.22 & 71.70 \\
% 			CoOp~\cite{COOP}   &77.58  &73.11  &75.28   \\
% 			\midrule
% 			VPT~\cite{jia2022visual}   &72.53  &72.34  &72.43   \\
%                \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &{74.98}  &{74.97}  &{75.03}  \\
% 			\midrule
%                    CoCoOp~\cite{cocoop} &{80.47} & 71.69 &75.83 \\
%                                 \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &{81.35}  &{74.97}  &{77.72}  \\
% 			\midrule
%          MaPLe~\cite{khattak2023maple} & 82.28 & {75.14} & {78.55}  \\
%                       \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &\color{blue}\textbf{{83.39}}  &\color{blue}\textbf{77.32}  &\color{blue}\textbf{80.36}   \\         
% 			\bottomrule
% 		\end{tabular}}
% 	\end{subtable}
% 	\vspace{-1mm}
% 	\begin{subtable}[t]{.32\textwidth}
% 		\centering
% 		\caption{ImageNet.}
% 		    \scalebox{.6}{
% 		\begin{tabular}{l cc|c}
% 			\toprule
% 			& Base & New & H \\
% 			\midrule
% 			CLIP~\cite{radford2021learning} & 72.43 & 68.14 & 70.22 \\
%    			CoOp~\cite{COOP}   &76.21 &69.98   &72.96   \\
% 			\midrule
% 			VPT~\cite{jia2022visual}   &74.45  &69.22  &71.74   \\
%            \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &{74.97}  &{69.99}  &{72.97}   \\
% 			\midrule
%    			CoCoOp~\cite{cocoop} & 75.98 &70.43 &73.10 \\
%               \rowcolor{lightGray}
% 			{+ {Prompt Diffusion}}   &{76.46}  &{70.97} &{73.36}   \\
% 			\midrule
%     MaPLe~\cite{khattak2023maple} & {76.66} & {70.54} & {73.47} \\
%             \rowcolor{lightGray}
%     			{+ {Prompt Diffusion}}   & \color{blue}\textbf{77.01}  &\color{blue}\textbf{71.03}  &\color{blue}\textbf{74.25}   \\
% 			\bottomrule
% 		\end{tabular}}
% 	\end{subtable}
% 	~\vspace{-1mm}
% 	\begin{subtable}[t]{.32\textwidth}
% 		\centering
% 		\caption{Caltech101.}
% 		    \scalebox{.6}{
% 		\begin{tabular}{l cc|c}
% 			\toprule
% 			& Base & New & H \\
% 			\midrule
% 			CLIP~\cite{radford2021learning} & 96.84 &94.00 & 95.40 \\
%    			CoOp~\cite{COOP}    &97.49   &94.67   &96.06   \\
% 			\midrule 
% 			VPT~\cite{jia2022visual}   &96.92  &93.44  &95.15   \\
% 			 \rowcolor{lightGray} {+ {Prompt Diffusion}}  &{97.43}  &{94.23}  &{95.83}    \\
% 			\midrule
%       			CoCoOp~\cite{cocoop} & 97.96 & 93.81 & 95.84 \\
% 			 \rowcolor{lightGray} {+ {Prompt Diffusion}}   &\color{blue}\textbf{98.12} &{94.97}  &{96.48}   \\
% 			\midrule
%     MaPLe~\cite{khattak2023maple} & 97.74 & {94.36} & {96.02} \\
%     			 \rowcolor{lightGray} {+ {Prompt Diffusion}}   &{97.25}  & \color{blue}\textbf{95.98}  &\color{blue}\textbf{96.81}   \\
% 			\bottomrule
% 		\end{tabular}}
% 	\end{subtable}

%   \label{tab:base2new}
% \end{table}





==> tables/cross-dataset_4.tex <==
\begin{table*}[!t]
	\tabstyle{5pt}
\caption{\textbf{Cross-dataset Generalization:} Accuracy (\%) evaluation for prompts learned from the source dataset (16-shots). Our model, when combined with various prompt learning methods, outperforms the baseline methods across multiple datasets.}

	\vspace{-0.1cm}
	\label{ap_t2}
    \scalebox{0.85}{
	\begin{tabular}{l c ccccccccccc}
		\toprule
		& Source & \multicolumn{11}{c}{Target} \\ \cmidrule(lr){2-2} \cmidrule(lr){3-13}
		& \rotatebox{45}{ImageNet} & \rotatebox{45}{Caltech101} & \rotatebox{45}{OxfordPets} & \rotatebox{45}{StanfordCars} & \rotatebox{45}{Flowers102} & \rotatebox{45}{Food101} & \rotatebox{45}{Aircraft} & \rotatebox{45}{SUN397} & \rotatebox{45}{DTD} & \rotatebox{45}{EuroSAT} & \rotatebox{45}{UCF101} & \rotatebox{45}{Average} \\
		\midrule
		CoOp  &69.86 &93.70	&89.14	&64.51	&68.71	&85.30	&18.47	&64.15	&41.92	&45.39	&66.55	&63.78\\		
		\midrule

		CoCoOp   &70.13 &93.33	&88.76	&64.49	&69.00	&85.48	&19.09	&64.03	&42.58	&45.61	&66.43	&63.88\\
		\textbf{{+ Ours}} &{70.49}		&\color{blue}\textbf{94.97}	&\color{blue}\textbf{91.25}	&{65.13}	&{69.63}	&{86.01}	&{20.17}	&{64.97}	&{41.71}	&{46.92}	&{67.13}	&{64.94}\\
		
		\midrule
		VPT &70.11	&93.30	&87.76	&62.64	&67.91	&83.64	&20.62	&64.51	&41.21	&40.85	&63.37	&62.58\\
		
		\textbf{{+ Ours}} &{70.81}		&{94.17}	&{88.52}	&{63.92}	&{68.03}	&{83.73}	&{21.82}	&{64.72}	&{42.17}	&{41.92}	&{63.77}	&{63.25}\\
		% \midrule
  %   	MaPLe & 70.72 & 93.53 & {90.49} & {65.57} & {72.23} & {86.20} & {24.74} & 67.01 & {46.49} & {48.06} & \color{blue}\textbf{68.69} & {66.30} \\
		% \textbf{{+ Ours}} & \color{blue}\textbf{71.23} & 93.98 & {91.11} & \color{blue}\textbf{66.17} & \color{blue}\textbf{73.13} & \color{blue}\textbf{87.14} & \color{blue}\textbf{25.23} & \color{blue}\textbf{68.03} & \color{blue}\textbf{46.95} & \color{blue}\textbf{48.73} & {68.53} & \color{blue}\textbf{67.70} \\

		\bottomrule
	\end{tabular}}
\vspace{-4mm}
\end{table*}

==> tables/domain_generalization.tex <==
\begin{table}[!t]
    \scalebox{0.8}{
	\begin{tabular}{l cccccc}
		\toprule
		& Source & \multicolumn{5}{c}{Target} \\ \cmidrule(lr){2-2} \cmidrule(lr){3-7}
		& ImageNet & -V2 & -S & -A & -R &Average\\
		\midrule
		CLIP  & 66.73 & 60.83 & 46.15 & 47.77 & 73.96  &57.18\\
		CoOp   &71.35          &64.28           &48.67        &50.65            &76.50       &60.03     \\
		\midrule
  				VPT  &  68.92   &61.84  &47.64  &46.50   &75.86    &57.96            \\
		            \rowcolor{lightGray} \textit{{+ Ours}}  &{70.23}        &{62.97}           &{48.77}            &{47.25}  &{77.06} &{59.24} \\
		\midrule
  CoCoOp  & 71.02 & 64.07 & 48.75 &50.63 &76.18 &59.91\\
		            \rowcolor{lightGray} \textit{{+ Ours}} & \color{blue}\textbf{71.98}        & {65.03}           &{49.86}            &\color{blue}\textbf{51.98}   &{77.25} &{61.25} \\
		\midrule
		{MaPLe} & 70.72 & {64.07} &{49.15} & {50.90}  & {76.98}  & {60.83}  \\
  		            \rowcolor{lightGray} \textit{{+ Ours}}  &{ 71.23}        &\color{blue}\textbf{65.24}           &\color{blue}\textbf{50.21}            &{51.93}  &\color{blue}\textbf{78.06} &\color{blue}\textbf{62.11} \\
		\bottomrule 
	\end{tabular}}
 \caption{\textbf{Domain generalization.} Accuracy (\%) evaluation on target datasets using prompts learned from a source dataset. Our method demonstrates consistent improvements across all datasets.}
 \vspace{-10mm}
\label{tab:dg}
\end{table}

==> tables/generative.tex <==
\begin{table}
\centering
\scalebox{0.95}{
	\begin{tabular}{l cc|c}
			\toprule
			& Base & New & H \\
			\midrule
                CoCoOp~\cite{cocoop} &{80.47} & 71.69 &75.83 \\
                \midrule
                w/MLP &{79.18} & 71.98 &75.91 \\
                w/Transformer &{80.17} & 72.03 &75.99 \\
                \midrule
                w/VAE &{80.73} & 72.09 &76.22 \\
                w/Normalizing flows &{80.65} & 72.43 & 76.35 \\
                % Bayesian prompt learning~\cite{derakhshani2023bayesian} & - & 74.69 &- \\
            \rowcolor{lightGray}
			{ \textbf{w/ Diffusion} }   & \color{blue}\textbf{81.35}  & \color{blue}\textbf{74.97}  &\color{blue}\textbf{77.72}   \\   
			\bottomrule
		\end{tabular}}
  \caption{\textbf{Benefit of diffusion model} in the base-to-new generalization. Our diffusion prompting method exceeds the efficacy of both generative and non-generative alternatives. }
  \vspace{-8mm}
\label{tab:generative}
\end{table}

==> tables/kd_cosine.tex <==
\begin{table}[t]
\begin{minipage}[t]{0.45\textwidth}
    \makeatletter\def\@captype{table}
    \centering
    \tabstyle{3pt}
    \caption{Comparison with knowledge distillation. Average accuracy (\%) over 11 datasets.}
    \vspace{2mm}
    \label{tab:compare_kd}
    \begin{tabular}{l ccccc}
    \toprule
    \#shots & 1 & 2 & 4 & 8 & 16 \\
    \midrule
    CoOp & 59.46 & 62.37 & 66.79 &  70.04 &  73.49 \\
     + KD  & 61.52  & 64.07 & 66.52 & 70.01 & 72.01 \\
     + ProGrad & \textbf{62.61} & \textbf{64.90} & \textbf{68.45} & \textbf{71.41} & \textbf{73.95}\\
    \bottomrule
    \end{tabular}
\end{minipage}
\hspace{1em}
\begin{minipage}[t]{0.45\textwidth}
    \makeatletter\def\@captype{table}
    \centering
    \tabstyle{3pt}
    \caption{Applying ProGrad to cosine classifier. Average accuracy (\%) over 11 datasets.}
    \vspace{2mm}
    \label{tab:compare_ProGrad}
    \begin{tabular}{l ccccc}
    \toprule
    \#shots & 1 & 2 & 4 & 8 & 16 \\
    \midrule
    Cosine & 30.50& 43.74& 53.33 & 61.26 & 65.00 \\
     + ProGrad & \textbf{32.29} & \textbf{46.14}&\textbf{55.18} & \textbf{62.05} & \textbf{66.47}\\
    \bottomrule
    \end{tabular}
\end{minipage}
\vspace{-4mm}
\end{table}


==> tables/training_time.tex <==
\setlength\intextsep{0pt}
\begin{wraptable}{r}{0.5\textwidth}
\centering
\caption{Training time comparison. Time is normalized to make training time of CoOp to 1.}\label{tab:time}
\scalebox{0.85}{
\begin{tabular}{lccc}
\toprule
Method            & CoOp & \texttt{ProGrad} & CoCoOp            \\ \midrule
Normalized Time   & 1.0  &  1.2 & 39.5 \\
\bottomrule
\end{tabular}
}
\end{wraptable}
